LaTr: Layout-Aware Transformer for Scene-Text VQA

We propose a novel multimodal architecture for Scene Text Visual Question Answering (STVQA), named Layout-Aware Transformer (LaTr). The task of STVQA requires models to reason over different modalities. Thus, we first investigate the impact of each modality, and reveal the importance of the language module, especially when enriched with layout information. Accounting for this, we propose a single objective pre-training scheme that requires only text and spatial cues. We show that applying this pre-training scheme on scanned documents has certain advantages over using natural images, despite the domain gap. Scanned documents are easy to procure, text-dense and have a variety of layouts, helping the model learn various spatial cues (e.g. left-of, below etc.) by tying together language and layout information. Compared to existing approaches, our method performs vocabulary-free decoding and, as shown, generalizes well beyond the training vocabulary. We further demonstrate that LaTr improves robustness towards OCR errors, a common reason for failure cases in STVQA. In addition, by leveraging a vision transformer, we eliminate the need for an external object detector. LaTr outperforms state-of-the-art STVQA methods on multiple datasets. In particular, +7.6% on TextVQA, +10.8% on ST-VQA and +4.0% on OCR-VQA (all absolute accuracy numbers).

==> tables/TextVQA_rosetta.tex <==
% \begin{table}[t]
% \centering
% % split the table into two with and without Rosetta
% \begin{tabular}{ l c c }
%     \hline
%     Method & Val Acc. & Test Acc.\\
%     \hline
%     LoRRA~\cite{singh2019towards} & 26.56 & 27.63 \\
%     MM-GNN~\cite{gao2020multi} & 31.44 & 31.10 \\
%     M4C~\cite{hu2020iterative} & 39.40 & 39.01 \\
%     SMA~\cite{gao2020structured} & 40.05 & 40.66 \\
%     CRN~\cite{liu2020cascade} & 40.39 & 40.96 \\
%     LaAP-Net~\cite{han2020finding} & 40.68 & 40.54 \\
%     % \rowcolor{LightGray}
%     % \AlgoName~(Ours) (No visual) & \eat{\zyang{44.06}}44.12 & - \\
%     % \AlgoName~(Ours) (No visual)& 70M Doc. & \eat{\zyang{48.08}}48.08 & - \\
%     M4C~\cite{hu2020iterative} & 40.55 & 40.46 \\
%     LaAP-Net~\cite{han2020finding} &  41.02 & 40.54 \\
%     % M4C$^\dagger$~\cite{hu2020iterative}   & 39.55 & - \\
%     TAP~\cite{yang2021tap} & \eat{\zyang{44.06}}44.06 & - \\
%     \rowcolor{LightGray} \AlgoNameSpace-Base  & 44.06  & - \\
%     \rowcolor{LightGray} \AlgoNameSpace$^*$-Base  &  \textbf{48.38} & - \\
% \end{tabular}
% \caption{Results on the TextVQA dataset~\cite{singh2019towards} with Rosetta OCR system. $^*$ refers to the model pretrained on 70M documents.}
% \vspace{-0.1in}
% \label{table:textvqa_rosetta}
% \end{table}


\begin{table}
\normalsize
\begin{center}
\small
\bgroup
\def\arraystretch{1.1}
        \begin{tabular}{lcc}
        \toprule
        Method & Val Acc. & Test Acc.\\
        \midrule
        LoRRA~\cite{singh2019towards} & 26.56 & 27.63 \\
        MM-GNN~\cite{gao2020multi} & 31.44 & 31.10 \\
        M4C~\cite{hu2020iterative} & 39.40 & 39.01 \\
        SMA~\cite{gao2020structured} & 40.05 & 40.66 \\
        CRN~\cite{liu2020cascade} & 40.39 & 40.96 \\
        LaAP-Net~\cite{han2020finding} & 40.68 & 40.54 \\
        % \rowcolor{LightGray}
        % \AlgoName~(Ours) (No visual) & \eat{\zyang{44.06}}44.12 & - \\
        % \AlgoName~(Ours) (No visual)& 70M Doc. & \eat{\zyang{48.08}}48.08 & - \\
        M4C~\cite{hu2020iterative} & 40.55 & 40.46 \\
        LaAP-Net~\cite{han2020finding} &  41.02 & 40.54 \\
        % M4C$^\dagger$~\cite{hu2020iterative}   & 39.55 & - \\
        TAP~\cite{yang2021tap} & \eat{\zyang{44.06}}44.06 & - \\
        \rowcolor{LightGray} \AlgoNameNoSpace-Base  & 44.06  & - \\
        \rowcolor{LightGray} \AlgoNameNoSpace$^*$-Base  &  \textbf{48.38} & - \\
        \bottomrule
    \end{tabular}
\egroup
\tiny
\caption{Results on the TextVQA dataset~\cite{singh2019towards} with Rosetta OCR system. $^*$ refers to the model pretrained on 70M documents.}
\label{table:textvqa_rosetta}
\end{center}
\end{table}
